Cross-Validation and Uncertainty Determination for Randomized Neural Networks with Applications to Mobile Sensors

Randomized artificial neural networks such as extreme learning machines provide an attractive and efficient method for supervised learning under limited computing ressources and green machine learning. This especially applies when equipping mobile devices (sensors) with weak artificial intelligence. Results are discussed about supervised learning with such networks and regression methods in terms of consistency and bounds for the generalization and prediction error. Especially, some recent results are reviewed addressing learning with data sampled by moving sensors leading to non-stationary and dependent samples. As randomized networks lead to random out-of-sample performance measures, we study a cross-validation approach to handle the randomness and make use of it to improve out-of-sample performance. Additionally, a computationally efficient approach to determine the resulting uncertainty in terms of a confidence interval for the mean out-of-sample prediction error is discussed based on two-stage estimation. The approach is applied to a prediction problem arising in vehicle integrated photovoltaics.

==> arxiv-version/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
%%%\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
%%%\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
%%%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}

%
% Monograph
%%%\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
%journal article
\bibitem{Ardot2010} Arlot, S., and Celisse, A. A survey of cross-validation procedures for model selection. Statist. Surv. \textbf{4}, 40--79, 2010.\\
doi:10.1214/09-SS054. 
% Journal article
\bibitem{Barron1993} Barron, A.R. Universal approximation bounds for superposition of a sigmoidal function. IEEE Trans. on Information Theory \textbf{39}, 3, 930--945, 1993. 
% journal
\bibitem{Birnie2016VIPV} Birnie, D.P.. Analysis of energy capture by vehicle solar roofs in conjunction with workplace plug-in charging, Solar Energy \textbf{125}, 219--226, 2016.
% contribution in proceeding
\bibitem{AdamConv2019} Bock, S. and Weiss, M. (2019). A proof of local convergence for the Adam optimizer. In: IEEE International Joint Conference on Neural Networks (IJCANN), 2019, IEEE, New York.\\
\url{https://opus4.kobv.de/opus4-oth-regensburg/frontdoor/deliver/index/docId/50/file/IJCNN2019.pdf}
% Book
\bibitem{BG2011} B\"uhlmann, P. and van de Geer, S.: Statistics for high-dimensional data, Springer Series in Statistics, Springer, Heidelberg, 2011.
%journal
\bibitem{ChangSteland2020} Steland, A. and Chang, Y.T. High-confident nonparametric fixed-width uncertainty intervals and applications to projected high-dimensional data and common mean estimation, Sequential Analysis, in press, 2020.
% online doc
\bibitem{eMNIST2017} Cohen, G., Afshar, S., Tapson, J.  and Schaik, A. EMNIST: an extension of MNIST to handwritten letters, arXiv 1702.05373,
% Journal article
\bibitem{GabanEtAl2016} Gaban, A.N., Tyukin, I.Y., Prokhorov, D.V. and Sofeikov, K.I. Approximation with random bases: Pro et contra. Information Sciences, \textbf{364-365}, 129-145, 2016.
% Book
\bibitem{GKKW2002} Gy\"orfi, L., Kohler, M., Krzyzak, A. and Walk, H. A Distribution-Free Theory of Nonparametric Regression. Springer Series in Statistics, Springer, New York, 2002.
% journal article
\bibitem{Delgao2014} Fern{{\'a}}ndez-Delgadom M., Cernadas, E., Barro, S. and  Amorim, D. Do we need hundreds of classifiers to solve real world classification problems? Journal of Machine Learning Research \textbf{15}(90), 3133-3181, 2014.
% journal article
\bibitem{Huang2004} Huang, G.-B., Zhu, Q.-Y. and Sieq, C.-K. Extreme learning machine: a new learning scheme of feedforward neural networks. IEEE International Joint Conference on Neural Networks, 985--990, 2004.
%journal
\bibitem{Silva2014} Lita da Silva, J. Some strong consistency results in stochastic regression. J. Multivariate Anal. \textbf{129}, 220--226, 2014.
% journal article
\bibitem{Huang2016} Tang, J., Deng, C. and Huang, G.-B. Extreme learning machine for multilayer perceptron. IEEE Transactions on Neural Networks and Learning Systems \textbf{27}(4), 809-821, 2016.
% Journal article
\bibitem{IgelnikPao1995} Igelnik, B. and Pao, Y.H. Stochastic choice of basis functions in additive function approximation and the functional-link net. IEEE Trans. on Neural Networks \textbf{6}(6), 1320--1329, 1995.
% Online doc
\bibitem{Adam2017} Kingma, D.P. and Ba, J.: Adam: A method for stochastic optimization. (2017). \\
\url{https://arxiv.org/abs/1412.6980. Cited 27 October 2020}
% journal article
\bibitem{Kuehnel2017VIPV} K\"uhnel, M., Hanke, B., Geissend\"orfer, S., von Maydell, K. and Agert, C. Energy forecast for mobile photovoltaic systems with focus on trucks for cooling applications. Progress in Photovoltaics: Research and Applications \textbf{25}(7), 525--532, 2017.
%journal
\bibitem{LiuYu2013} Liu, H. and Yu, Bin. Asymptotic properties of {L}asso+m{LS} and {L}asso+{R}idge in sparse high-dimensional linear regression. Electron. J. Stat. \textbf{7}, 3124--3169, 2013. 
% contribution in proceedings
\bibitem{BackProp2012} LeCun Y.A., Bottou L., Orr G.B. and M\"uller K.R. Efficient BackProp. In: Montavon G., Orr G.B., M\"uller KR. (eds) Neural Networks: Tricks of the Trade. Lecture Notes in Computer Science, vol 7700. Springer, Berlin, Heidelberg, 2012\\ \url{https://doi.org/10.1007/978-3-642-35289-8\_3}
% Journal article
\bibitem{LiuEtAl2015} Liu, X. and Lin, S. and Fang, J. and Xu, Z. Is extreme learning machine feasible? {A} theoretical assessment ({P}art {I}). IEEE Trans. Neural Netw. Learn. Syst. \textbf{26}, 7--20, 2015.
%Book
\bibitem{MohriRostaTal2018} Mohri, M., Rostamizadeh, A., and Talwalkar, A. Foundations of Machine Learning. 2nd ed, MIT Press, Cambridge, MA, 2018.
% contributinon
\bibitem{N2018} Neyshabur, B.,  Li, Z., Bhojanapalli, S., LeCun, Y., and  Srebro, N. The role of over-parametrization in generalization of neural networks. International Conference on Learning Representations, 2019.\\	
\url{https://openreview.net/forum?id=BygfghAcYX},
% journal article
\bibitem{SW2017} Scardapane, S. and Wang D. Randomness in neural networks: an overview, Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery \textbf{7}(2), 1--42, 2017.
% contribution conf
\bibitem{SchmidtEtAl1992} Schmidt, W.F., Kraaijveld, M.A. and Duin, R.P.W. Feedforward neural networks with random weights,  Proceedings of 11th IAPR International Conference on Pattern Recognition, Conference B: Pattern Recognition Methodology and Systems, \textbf{2}, 1--4, 1992.
%journal
\bibitem{SH2020} Schmidt-Hieber, J. Nonparametric regression using deep neural networks with ReLU activation function. Ann. Statist. \textbf{48}(4), 1875--1897, 2020.\\ doi:10.1214/19-AOS1875.
%journal article
\bibitem{Steland2012} Steland, A. Sequential data-adaptive bandwidth selection by vross-validation for nonparametric prediction. Communications in Statistics - Simulation and Computation \textbf{41}(7), 1195--1219, 2012.\\
doi: 10.1080/03610918.2012.625853
% online doc
\bibitem{Steland2020} Steland, A.: Extreme learning and regression for objects moving in non-stationary spatial environments, preprint on arXiv, 2020.\\
\url{https://arxiv.org/abs/2005.11115}
% under preparation
\bibitem{Steland2020b} Steland, A.: On consistency of cross-validation for randomized (deep) learners, under preparation, 2020.
% journal article
\bibitem{Stone1974} Stone, M. Cross-validatory choice and assessment of statistical predictions (with discussion). J. Roy. Statist. Soc. Ser. B \textbf{8}, 111--147, 1974.
% Journal article
\bibitem{Yang2007} Yang, Y.: Consistency of cross validation for comparing regression procedures. Ann. Statist. \textbf{35}, 2450--2473 (2007)
%
% Journal article by DOI
%%%\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
%\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
%%%\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
%%%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
%%%\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
%%%\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
%%%\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
%%%\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
\end{thebibliography}

